Binary quantization using Belief Propagation with decimation over factor graphs of LDGM codes

We propose a new algorithm for binary quantization based on the Belief Propagation algorithm with decimation over factor graphs of Low Density Generator Matrix (LDGM) codes. This algorithm, which we call Bias Propagation (BiP), can be considered as a special case of the Survey Propagation algorithm proposed for binary quantization by Wainwright et al. [8]. It achieves the same near-optimal rate-distortion performance with a substantially simpler framework and 10-100 times faster implementation. We thus challenge the widespread belief that binary quantization based on sparse linear codes cannot be solved by simple Belief Propagation algorithms. Finally, we give examples of suitably irregular LDGM codes that work with the BiP algorithm and show their performance.

==> fig_dd_conv_analysis.tex <==
\begin{figure}[t]
	\begin{center}
		\psfrag{title2}[bc][Bc]{\small Convergence condition $\convcond(\ddens{b}_\vect{s}, \rho^{(1-\tau)}, \lambda)$}
		%X axis
		\psfrag{X0}[tc][tc]{\footnotesize 0} \psfrag{X1}[tc][tc]{\footnotesize 0.1} \psfrag{X2}[tc][tc]{\footnotesize 0.2}
		\psfrag{X3}[tc][tc]{\footnotesize 0.3} \psfrag{X4}[tc][tc]{\footnotesize 0.4} \psfrag{X5}[tc][tc]{\footnotesize 0.5}
		\psfrag{X6}[tc][tc]{\footnotesize 0.6} \psfrag{X7}[tc][tc]{\footnotesize 0.7} \psfrag{X8}[tc][tc]{\footnotesize 0.8}
		\psfrag{X9}[tc][tc]{\footnotesize 0.9} \psfrag{X10}[tc][tc]{\footnotesize 1}
		%Y axis
		\psfrag{0}[Br][Br]{\footnotesize $0$} \psfrag{0.5}[Br][Br]{\footnotesize 0.5} \psfrag{0.2}[Br][Br]{\footnotesize 0.2} \psfrag{0.4}[Br][Br]{\footnotesize 0.4} \psfrag{0.6}[Br][Br]{\footnotesize 0.6} \psfrag{0.8}[Br][Br]{\footnotesize 0.8} \psfrag{1}[Br][Br]{\footnotesize 1} \psfrag{1.5}[Br][Br]{\footnotesize 1.5} \psfrag{2}[Br][Br]{\footnotesize 2} \psfrag{2.5}[Br][Br]{\footnotesize 2.5}
		\psfrag{xlabel}[tc][bc]{\small $(1-\tau)$ - ratio of removed info bits (percent)}
		\psfrag{ylabel2}[bc][tc]{} %\small $\convcond(\ddens{b}_\vect{s}, \rho(t), \lambda(t))$
		\psfrag{rho-1xxx}{\footnotesize $\rho_1(t)$} \psfrag{rho-2xxx}{\footnotesize $\rho_2(t)$} \psfrag{rho-3xxx}{\footnotesize $\rho_3(t)$} \psfrag{rho-4xxx}{\footnotesize $\rho_4(t)$}
		\includegraphics[viewport= 90 10 880 300, width=14cm, clip]{./figures/dd_conv_analysis.eps}
	\end{center}

	\caption{Convergence condition graph of regular (4,8) degree distribution (solid line) and irregular degree distribution of rate $R=0.5$ (dashed line) plotted for values $\gamma=0.9, 1, 1.1, 1.2$ (from top to bottom).}
	\label{fig:convergence-analysis}
\end{figure}

==> fig_results_weighted_case_dimension.tex <==
\begin{figure}

	{\begin{minipage}{11.3cm}
		%X axis
		\psfrag{X3}[cl]{\scriptsize $10^3$} \psfrag{X4}[cl]{\scriptsize $10^4$} \psfrag{X5}[cl]{\scriptsize $10^5$}
		%Y axis
		\psfrag{0.089}[Bl]{\scriptsize $\!\!\!\!$0.089}
		\psfrag{0.09}[Bl]{\scriptsize $\!\!\!\!$0.09}
		\psfrag{0.091}[Bl]{\scriptsize $\!\!\!\!$0.091}
		\psfrag{0.092}[Bl]{\scriptsize $\!\!\!\!$0.092}
		\psfrag{0.093}[Bl]{\scriptsize $\!\!\!\!$0.093}
		\psfrag{0.094}[Bl]{\scriptsize $\!\!\!\!$0.094}
		\psfrag{0.095}[Bl]{\scriptsize $\!\!\!\!$0.095}
		\psfrag{0.096}[Bl]{\scriptsize $\!\!\!\!$0.096}


		\psfrag{3000}[Bl]{\scriptsize $\!\!\!$3000}
		\psfrag{4000}[Bl]{\scriptsize $\!\!\!$4000}
		\psfrag{5000}[Bl]{\scriptsize $\!\!\!$5000}
		\psfrag{6000}[Bl]{\scriptsize $\!\!\!$6000}
		\psfrag{7000}[Bl]{\scriptsize $\!\!\!$7000}
		\psfrag{8000}[Bl]{\scriptsize $\!\!\!$8000}
		\psfrag{9000}[Bl]{\scriptsize $\!\!\!$9000}
		\psfrag{10000}[Bl]{\scriptsize $\!\!\!$10000}
		\psfrag{11000}[Bl]{\scriptsize $\!\!\!$11000}
		\psfrag{12000}[Bl]{\scriptsize $\!\!\!$12000}
		\psfrag{13000}[Bl]{\scriptsize $\!\!\!$13000}

		\psfrag{xlabel}[tl]{\small \hspace*{-1.7cm}$n$ - source sequence length}

		\psfrag{Throughput}[Bl]{\small \hspace*{-1.4cm}Throughput (bits/second)}
		\psfrag{Distortion}[Bl]{\small \hspace*{-1cm}Weighted distortion}

		\includegraphics[viewport=30 0 600 320, scale=0.6]{./results/dimension_lin_r0.5_q1_max_iter25_n100_26-Apr-2007_06-01-42.eps}
	\end{minipage}}
	\begin{minipage}{1cm} \footnotesize
		\vspace*{0cm}
		\begin{center} \begin{tabular}{|c|c|c|}
		\hline $n$ {\scriptsize $\cdot10^3$} & Dist. & Through. \\ \hline \hline
			1 & 0.0940 & 12444\\ \hline
			2 & 0.0922 & 10798\\ \hline
			3 & 0.0907 & 11237\\ \hline
			5 & 0.0901 & 10589\\ \hline
			7 & 0.0898 & 9915\\ \hline
			9 & 0.0898 & 9525\\ \hline
			10 & 0.0897 & 9294\\ \hline
			20 & 0.0890 & 8175\\ \hline
			30 & 0.0892 & 7393\\ \hline
			40 & 0.0891 & 6738\\ \hline
			50 & 0.0891 & 6099\\ \hline
			75 & 0.0890 & 4904\\ \hline
			100 & 0.0890 & 3873\\ \hline
		\end{tabular}\end{center}
	\end{minipage}
	\vspace*{0.3cm}

	\caption{Results from using weighted BiP algorithm for linear profile $\varrho$ using different code lengths, $R=0.5$. Values of $\gamma_a$ for each check node $a\in\checks$ were obtained using the polynomial fit from Figure~\ref{fig:results-weighted-case-gamma}.}
	\label{fig:results-weighted-case-dimension}
\end{figure}
